Implications of Mini-EUSO measurements for a space-based observation of UHECRs

Mini-EUSO is the first mission of the JEM-EUSO program on board the International Space Station. It was launched in August 2019 and it is operating since October 2019 being located in the Russian section (Zvezda module) of the station and viewing our planet from a nadir-facing UV-transparent window. The instrument is based on the concept of the original JEM-EUSO mission and consists of an optical system employing two Fresnel lenses of 25 cm each and a focal surface composed of 36 Multi-Anode Photomultiplier tubes, 64 channels each, for a total of 2304 channels with single photon counting sensitivity and an overall field of view of 44$\times$44$^\circ$. Mini-EUSO can map the night-time Earth in the near UV range (predominantly between 290 nm and 430 nm), with a spatial resolution of about 6.3 km and different temporal resolutions of 2.5 $\mu$s, 320 $\mu$s and 41 ms. Mini-EUSO observations are extremely important to better assess the potential of a space-based detector in studying Ultra-High Energy Cosmic Rays (UHECRs) such as K-EUSO and POEMMA. In this contribution we focus the attention on the results of the UV measurements and we place them in the context of UHECR observations from space, namely the estimation of exposure.

==> JEM-EUSO_Authors_July2023.tex <==
\newpage
\noindent
{\Large\bf Full Authors list: The JEM-EUSO Collaboration\\}
%{\scriptsize (author-list as of July 1st, 2023)} \hspace{0.6cm}
%{\scriptsize (version  \today{} \currenttime{})}
%\vspace*{0.5cm}

\begin{sloppypar}
{\small \noindent
S.~Abe$^{fq}$, 
J.H.~Adams Jr.$^{pd}$, 
D.~Allard$^{cb}$,
P.~Alldredge$^{pd}$,
L.~Anchordoqui$^{pe}$,
A.~Anzalone$^{eh,ed}$, 
E.~Arnone$^{ek,el}$,
M.~Bagheri$^{ph}$,
B.~Baret$^{cb}$,
D.~Barghini$^{el,ek}$,
M.~Battisti$^{ek,el,cb}$,
R.~Bellotti$^{ea,eb}$, 
A.A.~Belov$^{kb}$, 
M.~Bertaina$^{ek,el}$,
P.F.~Bertone$^{pf}$,
M.~Bianciotto$^{ek,el}$,
P.L.~Biermann$^{db}$,
F.~Bisconti$^{ei}$, 
C.~Blaksley$^{ft}$, 
S.~Blin-Bondil$^{cb}$, 
K.~Bolmgren$^{na}$,
S.~Briz$^{pb}$,
J.~Burton$^{pd}$,
F.~Cafagna$^{ea.eb}$, 
G.~Cambi\'e$^{ei,ej}$,
D.~Campana$^{ef}$, 
F.~Capel$^{de}$, 
R.~Caruso$^{ec,ed}$, 
M.~Casolino$^{ft,ei,ej}$,
C.~Cassardo$^{ek,el}$, 
A.~Castellina$^{ek,em}$,
K.~\v{C}ern\'{y}$^{bb}$,  
M.J.~Christl$^{pf}$, 
R.~Colalillo$^{ef,eg}$,
L.~Conti$^{en,ei}$, 
G.~Cotto$^{ek,el}$, 
H.J.~Crawford$^{pa}$, 
R.~Cremonini$^{el}$,
A.~Creusot$^{cb}$, 
A.~de Castro G\'onzalez$^{pb}$,  
C.~de la Taille$^{ca}$, 
R.~Diesing$^{pb}$,
P.~Dinaucourt$^{ca}$,
A.~Di Nola$^{eg}$,
A.~Ebersoldt$^{db}$,
T.~Ebisuzaki$^{ft}$,
J.~Eser$^{pb}$,
F.~Fenu$^{eo}$, 
S.~Ferrarese$^{ek,el}$,
G.~Filippatos$^{pc}$, 
W.W.~Finch$^{pc}$,
F. Flaminio$^{eg}$,
C.~Fornaro$^{en,ei}$,
D.~Fuhne$^{pc}$,
C.~Fuglesang$^{na}$, 
M.~Fukushima$^{fe}$, 
S.~Gadamsetty$^{ph}$,
D.~Gardiol$^{ek,em}$,
G.K.~Garipov$^{kb}$, 
E.~Gazda$^{ph}$, 
A.~Golzio$^{ek,el}$,
F.~Guarino$^{ef,eg}$, 
C.~Gu\'epin$^{pb}$,
A.~Haungs$^{db}$,
T.~Heibges$^{pc}$,
F.~Isgr\`o$^{ef,eg}$, 
E.G.~Judd$^{pa}$, 
F.~Kajino$^{ff}$, 
I.~Kaneko$^{ft}$, 
M.~Kleifges$^{db}$,
P.A.~Klimov$^{kb}$,
I.~Kreykenbohm$^{da}$, 
J.F.~Krizmanic$^{pj}$, 
V.~Kungel$^{pc}$,  
E.~Kuznetsov$^{pd}$, 
F.~L\'opez~Mart\'inez$^{pb}$, 
D.~Mand\'{a}t$^{bc}$,
M.~Manfrin$^{ek,el}$,
A. Marcelli$^{ej}$,
L.~Marcelli$^{ei}$, 
W.~Marsza{\l}$^{ia}$, 
J.N.~Matthews$^{pg}$, 
A.~Menshikov$^{db}$,
M.~Mese$^{ef,eg}$, 
S.S.~Meyer$^{pb}$,
J.~Mimouni$^{ad}$, 
H.~Miyamoto$^{ek,el}$, 
Y.~Mizumoto$^{fi}$,
A.~Monaco$^{ea,eb}$, 
S.~Nagataki$^{ft}$, 
J.~M.~Nachtman$^{pi}$,
D.~Naumov$^{ka}$,
A.~Neronov$^{cb}$,  
T.~Nonaka$^{fe}$, 
T.~Ogawa$^{ft}$, 
S.~Ogio$^{ft}$, 
H.~Ohmori$^{ft}$, 
A.V.~Olinto$^{pb}$,
Y.~Onel$^{pi}$,
G.~Osteria$^{ef}$,  
A.N.~Otte$^{ph}$,  
A.~Pagliaro$^{eh,ed}$,  
B.~Panico$^{ef, eg}$,  
E.~Parizot$^{cb, cd}$, 
I.H.~Park$^{gb}$, 
T.~Paul$^{pe}$,
M.~Pech$^{bc}$, 
F.~Perfetto$^{ef}$,  
P.~Picozza$^{ei,ej}$, 
L.W.~Piotrowski$^{ib}$,
Z.~Plebaniak$^{ei, ej}$, 
J.~Posligua$^{pi}$,
M.~Potts$^{ph}$,
R.~Prevete$^{ef,eg}$,
G.~Pr\'ev\^ot$^{cb}$,
M.~Przybylak$^{ia}$, 
E.~Reali$^{ei, ej}$,
P.~Reardon$^{pd}$, 
M.H.~Reno$^{pi}$, 
M.~Ricci$^{ee}$, 
O.F.~Romero~Matamala$^{ph}$, 
G.~Romoli$^{ei, ej}$,
H.~Sagawa$^{fe}$, 
N.~Sakaki$^{ft}$, 
A.~Santangelo$^{dd}$, 
O.A.~Saprykin$^{kc}$,
F.~Sarazin$^{pc}$,
M.~Sato$^{fo}$, 
H.~Schieler$^{db}$,
P.~Schov\'{a}nek$^{bc}$,
V.~Scotti$^{ef,eg}$,
S.~Selmane$^{cb}$
S.A.~Sharakin$^{kb}$,
K.~Shinozaki$^{ia}$, 
S.~Stepanoff$^{ph}$,
J.F.~Soriano$^{pe}$,
J.~Szabelski$^{ia}$,
N.~Tajima$^{ft}$, 
T.~Tajima$^{ft, pn}$,
Y.~Takahashi$^{fo}$, 
M.~Takeda$^{fe}$, 
Y.~Takizawa$^{ft}$, 
C.~Tenzer$^{dd}$,
S.B.~Thomas$^{pg}$, 
L.G.~Tkachev$^{ka}$,
T.~Tomida$^{fh}$, 
S.~Toscano$^{ob}$,  
M.~Tra\"{i}che$^{aa}$,  
D.~Trofimov$^{cb,kb}$,
K.~Tsuno$^{ft}$,  
P.~Vallania$^{ek,em}$,
L.~Valore$^{ef,eg}$,
T.~M.~Venters$^{pj}$,
C.~Vigorito$^{ek,el}$, 
M.~Vrabel$^{ia}$, 
S.~Wada$^{ft}$,  
J.~Watts~Jr.$^{pd}$, 
A.~Weindl$^{db}$,
L.~Wiencke$^{pc}$, 
J.~Wilms$^{da}$,
D.~Winn$^{pm}$,
H.~Wistrand$^{pc}$,
I.V.~Yashin$^{kb}$, 
R.~Young$^{pf}$,
M.Yu.~Zotov$^{kb}$.
}
\end{sloppypar}
\vspace*{.3cm}

%%\newpage
{ \footnotesize
\noindent
% Algeria - 2 institutes
$^{aa}$ Centre for Development of Advanced Technologies (CDTA), Algiers, Algeria \\
$^{ad}$ Lab. of Math. and Sub-Atomic Phys. (LPMPS), Univ. Constantine I, Constantine, Algeria \\
% Czech Republic - 2 institutes
$^{bb}$ Joint Laboratory of Optics, Faculty of Science, Palack\'{y} University, Olomouc, Czech Republic\\
$^{bc}$ Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic\\
% France - 3 institutes  
$^{ca}$ Omega, Ecole Polytechnique, CNRS/IN2P3, Palaiseau, France\\
$^{cb}$ Universit\'e de Paris, CNRS, AstroParticule et Cosmologie, F-75013 Paris, France\\
$^{cd}$ Institut universitaire de France (IUF)\\
% Germany - 4 institutes
$^{da}$ ECAP, University of Erlangen-Nuremberg, Germany\\
$^{db}$ Karlsruhe Institute of Technology (KIT), Germany\\
$^{dd}$ Institute for Astronomy and Astrophysics, Kepler Center, University of T\"ubingen, Germany\\
$^{de}$ Max Planck Institute for Physics, Munich, Germany\\
% Italy - 15 institutes  
$^{ea}$ Istituto Nazionale di Fisica Nucleare - Sezione di Bari, Italy\\
$^{eb}$ Universita' degli Studi di Bari Aldo Moro and INFN - Sezione di Bari, Italy\\
$^{ec}$ Dipartimento di Fisica e Astronomia "Ettore Majorana", Universita' di Catania, Italy\\
$^{ed}$ Istituto Nazionale di Fisica Nucleare - Sezione di Catania, Italy\\
$^{ee}$ Istituto Nazionale di Fisica Nucleare - Laboratori Nazionali di Frascati, Italy\\
$^{ef}$ Istituto Nazionale di Fisica Nucleare - Sezione di Napoli, Italy\\
$^{eg}$ Universita' di Napoli Federico II - Dipartimento di Fisica "Ettore Pancini", Italy\\
$^{eh}$ INAF - Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo, Italy\\
$^{ei}$ Istituto Nazionale di Fisica Nucleare - Sezione di Roma Tor Vergata, Italy\\
$^{ej}$ Universita' di Roma Tor Vergata - Dipartimento di Fisica, Roma, Italy\\
$^{ek}$ Istituto Nazionale di Fisica Nucleare - Sezione di Torino, Italy\\
$^{el}$ Dipartimento di Fisica, Universita' di Torino, Italy\\
$^{em}$ Osservatorio Astrofisico di Torino, Istituto Nazionale di Astrofisica, Italy\\
$^{en}$ Uninettuno University, Rome, Italy\\
$^{eo}$ Agenzia Spaziale Italiana, Via del Politecnico, 00133, Roma, Italy\\
% Japan - 7 institutes 
$^{fe}$ Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Japan\\ 
$^{ff}$ Konan University, Kobe, Japan\\ 
$^{fh}$ Shinshu University, Nagano, Japan \\
$^{fi}$ National Astronomical Observatory, Mitaka, Japan\\ 
$^{fo}$ Hokkaido University, Sapporo, Japan \\ 
$^{fq}$ Nihon University Chiyoda, Tokyo, Japan\\ 
$^{ft}$ RIKEN, Wako, Japan\\
% Korea - 1 institute
$^{gb}$ Sungkyunkwan University, Seoul, Republic of Korea\\
% Poland - 2 institutes
$^{ia}$ National Centre for Nuclear Research, Otwock, Poland\\
$^{ib}$ Faculty of Physics, University of Warsaw, Poland\\
% Russia - 3 institutes 
$^{ka}$ Joint Institute for Nuclear Research, Dubna, Russia\\
$^{kb}$ Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, Russia\\
$^{kc}$ Space Regatta Consortium, Korolev, Russia\\
% Sweden - 1 institute 
$^{na}$ KTH Royal Institute of Technology, Stockholm, Sweden\\
% Switzerland - 1 institute 
$^{ob}$ ISDC Data Centre for Astrophysics, Versoix, Switzerland\\
% USA - 12 institutes 
$^{pa}$ Space Science Laboratory, University of California, Berkeley, CA, USA\\
$^{pb}$ University of Chicago, IL, USA\\
$^{pc}$ Colorado School of Mines, Golden, CO, USA\\
$^{pd}$ University of Alabama in Huntsville, Huntsville, AL; USA\\
$^{pe}$ Lehman College, City University of New York (CUNY), NY, USA\\
$^{pf}$ NASA Marshall Space Flight Center, Huntsville, AL, USA\\
$^{pg}$ University of Utah, Salt Lake City, UT, USA\\
$^{ph}$ Georgia Institute of Technology, USA\\
$^{pi}$ University of Iowa, Iowa City, IA, USA\\
$^{pj}$ NASA Goddard Space Flight Center, Greenbelt, MD, USA\\
$^{pm}$ Fairfield University, Fairfield, CT, USA\\
$^{pn}$ Department of Physics and Astronomy, University of California, Irvine \\
}


==> JEM-EUSO_Authors_July2023_final.tex <==
\newpage
{\Large\bf Full Authors list: The JEM-EUSO Collaboration\\}
%{\scriptsize (author-list as of July 15th, 2023 with reorganized affiliations)} \hspace{0.6cm}
%{\scriptsize (version  \today{} \currenttime{})}
%\vspace*{0.5cm}

\begin{sloppypar}
{\small \noindent
S.~Abe$^{ff}$, 
J.H.~Adams Jr.$^{ld}$, 
D.~Allard$^{cb}$,
P.~Alldredge$^{ld}$,
R.~Aloisio$^{ep}$,
L.~Anchordoqui$^{le}$,
A.~Anzalone$^{ed,eh}$, 
E.~Arnone$^{ek,el}$,
M.~Bagheri$^{lh}$,
B.~Baret$^{cb}$,
D.~Barghini$^{ek,el}$,
M.~Battisti$^{cb,ek,el}$,
R.~Bellotti$^{ea,eb}$, 
A.A.~Belov$^{ib}$, 
M.~Bertaina$^{ek,el}$,
P.F.~Bertone$^{lf}$,
M.~Bianciotto$^{ek,el}$,
F.~Bisconti$^{ei}$, 
C.~Blaksley$^{fg}$, 
S.~Blin-Bondil$^{cb}$, 
K.~Bolmgren$^{ja}$,
S.~Briz$^{lb}$,
J.~Burton$^{ld}$,
F.~Cafagna$^{ea.eb}$, 
G.~Cambi\'e$^{ei,ej}$,
D.~Campana$^{ef}$, 
F.~Capel$^{db}$, 
R.~Caruso$^{ec,ed}$, 
M.~Casolino$^{ei,ej,fg}$,
C.~Cassardo$^{ek,el}$, 
A.~Castellina$^{ek,em}$,
K.~\v{C}ern\'{y}$^{ba}$,  
M.J.~Christl$^{lf}$, 
R.~Colalillo$^{ef,eg}$,
L.~Conti$^{ei,en}$, 
G.~Cotto$^{ek,el}$, 
H.J.~Crawford$^{la}$, 
R.~Cremonini$^{el}$,
A.~Creusot$^{cb}$,
A.~Cummings$^{lm}$,
A.~de Castro G\'onzalez$^{lb}$,  
C.~de la Taille$^{ca}$, 
R.~Diesing$^{lb}$,
P.~Dinaucourt$^{ca}$,
A.~Di Nola$^{eg}$,
T.~Ebisuzaki$^{fg}$,
J.~Eser$^{lb}$,
F.~Fenu$^{eo}$, 
S.~Ferrarese$^{ek,el}$,
G.~Filippatos$^{lc}$, 
W.W.~Finch$^{lc}$,
F. Flaminio$^{eg}$,
C.~Fornaro$^{ei,en}$,
D.~Fuehne$^{lc}$,
C.~Fuglesang$^{ja}$, 
M.~Fukushima$^{fa}$, 
S.~Gadamsetty$^{lh}$,
D.~Gardiol$^{ek,em}$,
G.K.~Garipov$^{ib}$, 
E.~Gazda$^{lh}$, 
A.~Golzio$^{ek,el}$,
F.~Guarino$^{ef,eg}$, 
C.~Gu\'epin$^{lb}$,
A.~Haungs$^{da}$,
T.~Heibges$^{lc}$,
F.~Isgr\`o$^{ef,eg}$, 
E.G.~Judd$^{la}$, 
F.~Kajino$^{fb}$, 
I.~Kaneko$^{fg}$,
S.-W.~Kim$^{ga}$,
P.A.~Klimov$^{ib}$,
J.F.~Krizmanic$^{lj}$, 
V.~Kungel$^{lc}$,  
E.~Kuznetsov$^{ld}$, 
F.~L\'opez~Mart\'inez$^{lb}$, 
D.~Mand\'{a}t$^{bb}$,
M.~Manfrin$^{ek,el}$,
A. Marcelli$^{ej}$,
L.~Marcelli$^{ei}$, 
W.~Marsza{\l}$^{ha}$, 
J.N.~Matthews$^{lg}$, 
M.~Mese$^{ef,eg}$, 
S.S.~Meyer$^{lb}$,
J.~Mimouni$^{ab}$, 
H.~Miyamoto$^{ek,el}$, 
Y.~Mizumoto$^{fd}$,
A.~Monaco$^{ea,eb}$, 
S.~Nagataki$^{fg}$, 
J.M.~Nachtman$^{li}$,
D.~Naumov$^{ia}$,
A.~Neronov$^{cb}$,  
T.~Nonaka$^{fa}$, 
T.~Ogawa$^{fg}$, 
S.~Ogio$^{fg}$, 
H.~Ohmori$^{fg}$, 
A.V.~Olinto$^{lb}$,
Y.~Onel$^{li}$,
G.~Osteria$^{ef}$,  
A.N.~Otte$^{lh}$,  
A.~Pagliaro$^{ed,eh}$,  
B.~Panico$^{ef,eg}$,  
E.~Parizot$^{cb,cc}$, 
I.H.~Park$^{gb}$, 
T.~Paul$^{le}$,
M.~Pech$^{bb}$, 
F.~Perfetto$^{ef}$,  
P.~Picozza$^{ei,ej}$, 
L.W.~Piotrowski$^{hb}$,
Z.~Plebaniak$^{ei,ej}$, 
J.~Posligua$^{li}$,
M.~Potts$^{lh}$,
R.~Prevete$^{ef,eg}$,
G.~Pr\'ev\^ot$^{cb}$,
M.~Przybylak$^{ha}$, 
E.~Reali$^{ei, ej}$,
P.~Reardon$^{ld}$, 
M.H.~Reno$^{li}$, 
M.~Ricci$^{ee}$, 
O.F.~Romero~Matamala$^{lh}$, 
G.~Romoli$^{ei, ej}$,
H.~Sagawa$^{fa}$, 
N.~Sakaki$^{fg}$, 
O.A.~Saprykin$^{ic}$,
F.~Sarazin$^{lc}$,
M.~Sato$^{fe}$, 
P.~Schov\'{a}nek$^{bb}$,
V.~Scotti$^{ef,eg}$,
S.~Selmane$^{cb}$,
S.A.~Sharakin$^{ib}$,
K.~Shinozaki$^{ha}$, 
S.~Stepanoff$^{lh}$,
J.F.~Soriano$^{le}$,
J.~Szabelski$^{ha}$,
N.~Tajima$^{fg}$, 
T.~Tajima$^{fg, ll}$,
Y.~Takahashi$^{fe}$, 
M.~Takeda$^{fa}$, 
Y.~Takizawa$^{fg}$, 
S.B.~Thomas$^{lg}$, 
L.G.~Tkachev$^{ia}$,
T.~Tomida$^{fc}$, 
S.~Toscano$^{ka}$,  
M.~Tra\"{i}che$^{aa}$,  
D.~Trofimov$^{cb,ib}$,
K.~Tsuno$^{fg}$,  
P.~Vallania$^{ek,em}$,
L.~Valore$^{ef,eg}$,
T.M.~Venters$^{lj}$,
C.~Vigorito$^{ek,el}$, 
M.~Vrabel$^{ha}$, 
S.~Wada$^{fg}$,  
J.~Watts~Jr.$^{ld}$, 
L.~Wiencke$^{lc}$, 
D.~Winn$^{lk}$,
H.~Wistrand$^{lc}$,
I.V.~Yashin$^{ib}$, 
R.~Young$^{lf}$,
M.Yu.~Zotov$^{ib}$.
}
\end{sloppypar}
\vspace*{.3cm}

%%\newpage
{ \footnotesize
\noindent
% Algeria - 2 institutes
$^{aa}$ Centre for Development of Advanced Technologies (CDTA), Algiers, Algeria \\
$^{ab}$ Lab. of Math. and Sub-Atomic Phys. (LPMPS), Univ. Constantine I, Constantine, Algeria \\
% Czech Republic - 2 institutes
$^{ba}$ Joint Laboratory of Optics, Faculty of Science, Palack\'{y} University, Olomouc, Czech Republic\\
$^{bb}$ Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic\\
% France - 3 institutes  
$^{ca}$ Omega, Ecole Polytechnique, CNRS/IN2P3, Palaiseau, France\\
$^{cb}$ Universit\'e de Paris, CNRS, AstroParticule et Cosmologie, F-75013 Paris, France\\
$^{cc}$ Institut Universitaire de France (IUF), France\\
% Germany - 2 institutes
$^{da}$ Karlsruhe Institute of Technology (KIT), Germany\\
$^{db}$ Max Planck Institute for Physics, Munich, Germany\\
% Italy - 16 institutes  
$^{ea}$ Istituto Nazionale di Fisica Nucleare - Sezione di Bari, Italy\\
$^{eb}$ Universit\`a degli Studi di Bari Aldo Moro, Italy\\
$^{ec}$ Dipartimento di Fisica e Astronomia "Ettore Majorana", Universit\`a di Catania, Italy\\
$^{ed}$ Istituto Nazionale di Fisica Nucleare - Sezione di Catania, Italy\\
$^{ee}$ Istituto Nazionale di Fisica Nucleare - Laboratori Nazionali di Frascati, Italy\\
$^{ef}$ Istituto Nazionale di Fisica Nucleare - Sezione di Napoli, Italy\\
$^{eg}$ Universit\`a di Napoli Federico II - Dipartimento di Fisica "Ettore Pancini", Italy\\
$^{eh}$ INAF - Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo, Italy\\
$^{ei}$ Istituto Nazionale di Fisica Nucleare - Sezione di Roma Tor Vergata, Italy\\
$^{ej}$ Universit\`a di Roma Tor Vergata - Dipartimento di Fisica, Roma, Italy\\
$^{ek}$ Istituto Nazionale di Fisica Nucleare - Sezione di Torino, Italy\\
$^{el}$ Dipartimento di Fisica, Universit\`a di Torino, Italy\\
$^{em}$ Osservatorio Astrofisico di Torino, Istituto Nazionale di Astrofisica, Italy\\
$^{en}$ Uninettuno University, Rome, Italy\\
$^{eo}$ Agenzia Spaziale Italiana, Via del Politecnico, 00133, Roma, Italy\\
$^{ep}$ Gran Sasso Science Institute, L'Aquila, Italy\\
% Japan - 7 institutes 
$^{fa}$ Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Japan\\ 
$^{fb}$ Konan University, Kobe, Japan\\ 
$^{fc}$ Shinshu University, Nagano, Japan \\
$^{fd}$ National Astronomical Observatory, Mitaka, Japan\\ 
$^{fe}$ Hokkaido University, Sapporo, Japan \\ 
$^{ff}$ Nihon University Chiyoda, Tokyo, Japan\\ 
$^{fg}$ RIKEN, Wako, Japan\\
% Korea - 2 institutes
$^{ga}$ Korea Astronomy and Space Science Institute\\
$^{gb}$ Sungkyunkwan University, Seoul, Republic of Korea\\
% Poland - 2 institutes
$^{ha}$ National Centre for Nuclear Research, Otwock, Poland\\
$^{hb}$ Faculty of Physics, University of Warsaw, Poland\\
% Russia - 3 institutes 
$^{ia}$ Joint Institute for Nuclear Research, Dubna, Russia\\
$^{ib}$ Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, Russia\\
$^{ic}$ Space Regatta Consortium, Korolev, Russia\\
% Sweden - 1 institute 
$^{ja}$ KTH Royal Institute of Technology, Stockholm, Sweden\\
% Switzerland - 1 institute 
$^{ka}$ ISDC Data Centre for Astrophysics, Versoix, Switzerland\\
% USA - 13 institutes 
$^{la}$ Space Science Laboratory, University of California, Berkeley, CA, USA\\
$^{lb}$ University of Chicago, IL, USA\\
$^{lc}$ Colorado School of Mines, Golden, CO, USA\\
$^{ld}$ University of Alabama in Huntsville, Huntsville, AL, USA\\
$^{le}$ Lehman College, City University of New York (CUNY), NY, USA\\
$^{lf}$ NASA Marshall Space Flight Center, Huntsville, AL, USA\\
$^{lg}$ University of Utah, Salt Lake City, UT, USA\\
$^{lh}$ Georgia Institute of Technology, USA\\
$^{li}$ University of Iowa, Iowa City, IA, USA\\
$^{lj}$ NASA Goddard Space Flight Center, Greenbelt, MD, USA\\
$^{lk}$ Fairfield University, Fairfield, CT, USA\\
$^{ll}$ Department of Physics and Astronomy, University of California, Irvine, USA \\
$^{lm}$ Pennsylvania State University, PA, USA \\
}


